Recovering Structural Organization in Noisy Correlation Networks Using Financial Systems as a Testbed

Empirical correlation matrices estimated from financial return time series are contaminated by statistical noise arising from finite sample size, obscuring genuine interactions among assets. We apply spectral decomposition to separate the empirical correlation matrix into a structured component associated with eigenvalues exceeding the Marchenko-Pastur bounds and a random component representing statistical noise. Using daily returns from the NIFTY 200, NIFTY 500, and S&P 500 over 2010-2022, we show that the structured component, constructed from only 10-16 eigenmodes, reproduces the main statistical properties of the full correlation matrix while removing most noise-dominated eigenmodes. Financial networks derived from the structured component exhibit significantly stronger and more stable core-periphery organization than networks constructed from the full or random matrices. Degree-preserving randomization, Kolmogorov-Smirnov, and Wasserstein distance tests confirm a clear statistical separation between structured and random components. We further show that structured networks display pronounced scale-free degree distributions in the Indian markets. As a practical application, portfolios constructed from peripheral assets of the denoised networks consistently outperform portfolios based on unfiltered correlations and standard benchmarks on a risk-adjusted basis, with robustness verified through Monte Carlo subsampling. These results demonstrate that spectral denoising effectively recovers meaningful network structure from noisy financial correlations.

==> Discussion.tex <==
\section*{Discussion}
\label{sec:overall_results}


==> discussion.tex <==
\section*{Discussion}

This study examines portfolio construction in Indian and U.S. equity markets using a network-based framework grounded in the core--periphery (CP) organization of denoised correlation networks. Unlike conventional portfolio strategies that rely on individual asset characteristics or exogenous economic classifications, the proposed approach exploits meso-scale structural information embedded in the return correlation matrix. By combining Random Matrix Theory (RMT) filtering with probabilistic CP profiling, the method isolates economically meaningful dependence patterns from noise and evaluates their relevance for out-of-sample portfolio performance.

A central empirical result is that portfolios constructed from the structured mode \(C^{\mathrm{STR}}\) consistently outperform those based on the full correlation matrix \(C^{\mathrm{FULL}}\), as well as standard benchmarks including the market portfolio \(\boldsymbol{\pi}^{\mathrm{MKT}}\), the highest-Sharpe selection strategy \(\boldsymbol{\pi}^{\mathrm{HSR}}\), and the random selection benchmark \(\boldsymbol{\pi}^{\mathrm{RND}}\). This finding is robust across portfolio sizes \(M \in \{10,20,30,40\}\), weighting schemes (uniform and Markowitz), and market universes (NIFTY 200, NIFTY 500, and S\&P 500). The results emphasize the importance of suppressing noise-driven correlations, which are known to distort covariance estimation and degrade portfolio optimization, particularly in high-dimensional settings.

From a network perspective, the superior performance of structured-mode portfolios can be attributed to the fact that \(C^{\mathrm{STR}}\) retains only eigenmodes that deviate from the RMT bounds \([\lambda_{-},\lambda_{+}]\), thereby capturing genuine collective market dynamics. In contrast, portfolios derived from \(C^{\mathrm{FULL}}\) implicitly incorporate spurious correlations arising from finite-sample effects. These findings provide empirical support for the view that relevant financial information is concentrated in a low-dimensional subspace of the correlation matrix, and that exploiting this structure leads to more stable and reliable portfolio decisions.

The comparison between core-based \(\boldsymbol{\pi}^{(s)}_c\) and periphery-based \(\boldsymbol{\pi}^{(s)}_p\) portfolios reveals a systematic and economically interpretable trade-off. Core portfolios are composed of stocks that are strongly embedded in the market’s dependence structure, reflecting their central role in transmitting market-wide fluctuations. As a result, they tend to exhibit higher average returns during relatively stable periods but also display greater sensitivity to systemic shocks. In contrast, periphery portfolios consist of stocks with weaker and more heterogeneous correlations, which translates into lower volatility and improved downside protection, particularly during periods of market stress such as the COVID-19 crisis. Importantly, this adaptive allocation between core and periphery assets emerges endogenously from the network structure, without relying on external regime indicators or ad hoc risk signals.

These patterns are robust across different market sizes and levels of market complexity. While expanding the investment universe from the NIFTY 200 to the NIFTY 500 and further to the S\&P 500 increases estimation noise and correlation density, the RMT-based denoising step effectively mitigates these effects. Consequently, the CP structures extracted from \(C^{\mathrm{STR}}\) remain sufficiently stable to guide stock selection even in large-scale equity markets. This robustness is particularly relevant for practical applications, where portfolio strategies must operate under evolving market composition and heterogeneous liquidity conditions.

The rolling-window, out-of-sample evaluation further demonstrates that the proposed strategy does not rely on static network features. Instead, CP profiles evolve over time, reflecting structural reorganization in response to major market events. The persistence of performance improvements across successive rebalancing windows indicates that the network-guided selection captures stable structural properties rather than transient statistical artifacts.

Compared with existing literature on network-based portfolio optimization, the contribution of this work lies not in the qualitative observation that diversification benefits arise from weakly correlated assets, but in demonstrating that such benefits can be systematically achieved through a probabilistic CP framework applied to denoised equity correlation networks. Unlike approaches based on minimum spanning trees, planar filtered graphs, or asset-class segmentation, the present method operates directly at the meso-scale level and is applicable within a single asset class. This makes it particularly suitable for equity markets, where cross-asset hedging opportunities may be limited.


Our findings are consistent with earlier evidence showing that assets located in the periphery of financial correlation networks tend to play a stabilizing role during periods of elevated systemic risk. In particular, previous studies employing filtered network representations, such as PMFG-based frameworks, report that optimal portfolios frequently allocate higher weights to peripheral assets characterized by weak correlations with the market core, especially during crisis phases \cite{pozzi2013spread, wang2024portfolio}. The underlying mechanism is commonly attributed to the reduced exposure of peripheral nodes to collective market fluctuations, which enhances diversification and downside protection. While existing studies document this behavior primarily in global multi-asset settings and often rely on asset-class composition or macroeconomic narratives for interpretation, the present work demonstrates that the same structural mechanism operates within equity markets alone. By extracting meso-scale core--periphery structures from denoised correlation matrices, we show that peripheral \emph{stocks} systematically contribute to improved risk-adjusted performance without invoking exogenous economic classifications. These results highlight that incorporating meso-scale network structure into portfolio construction provides a principled and robust alternative to traditional optimization techniques based solely on raw correlations.




%\section*{Discussion}

%This study advances the field of network-based portfolio optimization by integrating Random Matrix Theory (RMT) filtering with CP structures, enhancing the reliability of financial network representations. By removing random noise from empirical correlations, the proposed framework yields a more stable and interpretable CP organization, enabling improved asset selection and portfolio diversification.

%Beyond methodological contributions, this work highlights the broader potential of combining RMT and core-periphery structures for portfolio construction, offering a robust alternative to traditional correlation-based methods. Specifically, our main findings demonstrate that:

%\begin{enumerate}

   % \item The CP structure is consistently captured in both the structured and market modes than the full cross correlation method.
    
  %  \item Peripheral stocks selected from mode-based matrices exhibit greater stability than those selected from the full cross-correlation matrix, highlighting the practical relevance of filtered correlation networks.
    
   % \item Portfolios constructed from peripheral stocks identified via mode-based methods benchmark favorably against those derived from the full cross-correlation approach.
    
   % \item Mode-based portfolio strategies outperform the corresponding Markowitz benchmark.
    
   % \item Portfolios constructed from mode-based peripheral stocks outperform their corresponding core-based portfolio strategies.

   % \item Reducing noise in the correlation matrix highlights the importance of one or a few significant eigenvalues in the filtering process, while also substantially reducing the computational cost of network construction.

% \item Filtering the correlation matrix using eigenvalue decomposition reduces the computational time complexity compared to traditional filtering approaches such as PMFG or MST. 


%\end{enumerate}

%Our results suggest that mode-based methods provide an effective and computationally efficient approach for noise reduction in correlation matrices compared with network-based filtering methods such as PMFG or TMFG.(\textbf{Can you provide computational time of these algorithm?)}



%\section*{Future Directions}

%Several promising avenues remain open for future exploration:
%\begin{itemize}

%\item This study has been conducted using daily stock price data from both an emerging and a developed market. A natural extension would be to apply the proposed methodologies to high-frequency tick-by-tick data, which could be particularly useful for intraday trading strategies.

%\item A comparative analysis with advanced portfolio construction techniques, such as multi-factor models and regime-switching frameworks, could provide deeper insights into the robustness and adaptability of the proposed approach. In addition, incorporating volatility-based segmentation or time-varying network filtering may better capture dynamic market regimes.

%\item The detection of CP structures in hypergraphs has recently gained significant attention~\cite{tudisco2023core,papachristou2022core}. Extending the proposed framework to hypergraph-based representations is a compelling direction for future research. Hypergraphs can capture higher-order dependencies among multiple stocks beyond pairwise correlations, potentially revealing richer structural patterns that influence portfolio performance. Developing such extensions would strengthen both the theoretical foundations and practical relevance of network-based portfolio strategies, paving the way toward a comprehensive, noise-filtered, and structurally informed paradigm for financial decision-making.

%\end{itemize}



%\section*{Acknowledgements}

%The first author acknowledge financial support from the Kotak IISc AI–ML Centre (KIAC) at the Indian Institute of Science (IISc), Bangalore, India.

==> fig.tex <==



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[htbp]
\centering
\footnotesize
\caption{Performance comparison of equal-weighted portfolio strategies in terms of signal-to-noise ratio, average returns, and volatility for portfolio sizes $M = \{10, 20, 30, 40\}$ over the holding horizon of $T = 125$ days, using NIFTY 200 stocks. Clearly, on average, the proposed investment strategy (\(\pi^{STR}_p\))  is outperforming all other strategies.}
\label{tab:nifty_200_uniform}
\begin{tabular*}{0.75\textwidth}{@{\extracolsep{\fill}} lcccccc|c }
\toprule
\textbf{M} & 
\(\boldsymbol{\pi}^{FULL}_p\) & 
\(\boldsymbol{\pi}^{STR}_p\) & 
\(\boldsymbol{\pi}^{FULL}_c\) & 
\(\boldsymbol{\pi}^{STR}_c\) & 
\(\boldsymbol{\pi}^{HSR}\) & 
\(\boldsymbol{\pi}^{RND}\) & 
\textit{\(\boldsymbol{\pi}^{MKT}\)} \\
\midrule
\multicolumn{8}{c}{\scriptsize \textit{Signal-to-noise ratio}} \\
\midrule
10 & 0.6525 & 0.6042 & 0.1864 & 0.1841 & 0.4663 & 0.6493 & \textit{0.5088} \\
20 & 0.6827 & \textbf{0.7723} & 0.2108 & 0.1893 & 0.4755 & 0.5822 & \textit{0.5088} \\
30 & 0.7097 & \textbf{0.8054} & 0.2397 & 0.1974 & 0.4923 & 0.5481 & \textit{0.5088} \\
40 & 0.7187 & \textbf{0.8097} & 0.2733 & 0.2268 & 0.4921 & 0.5360 & \textit{0.5088} \\
\midrule
\multicolumn{8}{c}{\scriptsize \textit{Average Return}} \\
\midrule
10 & 0.0894 & 0.0813 & 0.0399 & 0.0386 & 0.0753 & 0.0915 & \textit{0.0712} \\
20 & 0.0873 & \textbf{0.0880} & 0.0424 & 0.0389 & 0.0721 & 0.0878 & \textit{0.0712} \\
30 & 0.0874 & \textbf{0.0922} & 0.0458 & 0.0386 & 0.0727 & 0.0770 & \textit{0.0712} \\
40 & 0.0876 & \textbf{0.0902} & 0.0501 & 0.0433 & 0.0718 & 0.0772 & \textit{0.0712} \\
\midrule
\multicolumn{8}{c}{\scriptsize \textit{Volatility}} \\
\midrule
10 & 0.1370 & \textbf{0.1345} & 0.2139 & 0.2096 & 0.1615 & 0.1409 & \textit{0.1400} \\
20 & 0.1278 & \textbf{0.1139} & 0.2011 & 0.2056 & 0.1517 & 0.1508 & \textit{0.1400} \\
30 & 0.1232 & \textbf{0.1145} & 0.1909 & 0.1955 & 0.1476 & 0.1405 & \textit{0.1400} \\
40 & 0.1219 & \textbf{0.1115} & 0.1834 & 0.1908 & 0.1459 & 0.1440 & \textit{0.1400} \\
\bottomrule
\end{tabular*}
\end{table}









%\section{NIFTY 500}
\begin{table}[htbp]
\centering
\footnotesize
\caption{Performance comparison of equal-weighted portfolio strategies in terms of signal-to-noise ratio, average returns, and volatility for portfolio sizes $M = \{10, 20, 30, 40\}$ over a holding horizon of $T = 125$ days, using NIFTY 500 stocks. Clearly, the proposed investment strategy (\(\pi^{STR}_p\))  is outperforming all other strategies.}
\label{tab:nifty_500_uniform}
\begin{tabular*}{0.75\textwidth}{@{\extracolsep{\fill}} lcccccc|c }
\toprule
\textbf{M} &
\(\boldsymbol{\pi}^{FULL}_p\) &
\(\boldsymbol{\pi}^{STR}_p\) &
\(\boldsymbol{\pi}^{FULL}_c\) &
\(\boldsymbol{\pi}^{STR}_c\) &
\(\boldsymbol{\pi}^{HSR}\) &
\(\boldsymbol{\pi}^{RND}\) &
\textit{\(\boldsymbol{\pi}^{MKT}\)} \\
\midrule
\multicolumn{8}{c}{\scriptsize \textit{Signal-to-noise ratio}} \\
\midrule
10 & 0.6941 & \textbf{0.7847} & 0.0949 & 0.0833 & 0.5132 & 0.4478 & \textit{0.5233} \\
20 & 0.7552 & \textbf{0.8625} & 0.1584 & 0.1498 & 0.5267 & 0.5241 & \textit{0.5233} \\
30 & 0.7702 & \textbf{0.8319} & 0.1650 & 0.1525 & 0.5321 & 0.5373 & \textit{0.5233} \\
40 & 0.7737 & \textbf{0.8060} & 0.1885 & 0.1841 & 0.5297 & 0.5574 & \textit{0.5233} \\
\midrule
\multicolumn{8}{c}{\scriptsize \textit{Average Return}} \\
\midrule
10 & 0.1065 & \textbf{0.1184} & 0.0201 & 0.0173 & 0.0867 & 0.0788 & \textit{0.0804} \\
20 & 0.1052 & \textbf{0.1161} & 0.0319 & 0.0300 & 0.0842 & 0.0848 & \textit{0.0804} \\
30 & 0.1035 & \textbf{0.1079} & 0.0330 & 0.0302 & 0.0835 & 0.0834 & \textit{0.0804} \\
40 & 0.1023 & \textbf{0.1048} & 0.0366 & 0.0356 & 0.0821 & 0.0800 & \textit{0.0804} \\
\midrule
\multicolumn{8}{c}{\scriptsize \textit{Volatility}} \\
\midrule
10 & 0.1629 & \textbf{0.1592} & 0.2206 & 0.2209 & 0.1788 & 0.1711 & \textit{0.1599} \\
20 & 0.1485 & \textbf{0.1438} & 0.2133 & 0.2137 & 0.1681 & 0.1613 & \textit{0.1599} \\
30 & 0.1428 & \textbf{0.1375} & 0.2107 & 0.2097 & 0.1641 & 0.1540 & \textit{0.1599} \\
40 & 0.1408 & \textbf{0.1383} & 0.2052 & 0.2056 & 0.1621 & 0.1430 & \textit{0.1599} \\
\bottomrule
\end{tabular*}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table}[htbp]
\centering
\footnotesize
\caption{Performance comparison of equal-weighted portfolio strategies in terms of signal-to-noise ratio, average returns, and volatility for portfolio sizes $M = \{10, 20, 30, 40\}$ over a holding horizon of $T = 125$ days, using S\&P 500 stocks. Clearly, the proposed investment strategy (\(\pi^{STR}_p\))  outperforms all other strategies in terms of average return, while remaining competitive in the other performance measures.}
\label{tab:sp_500_uniform}
\begin{tabular*}{0.75\textwidth}{@{\extracolsep{\fill}} lcccccc|c }
\toprule
\textbf{M} &
\(\boldsymbol{\pi}^{FULL}_p\) &
\(\boldsymbol{\pi}^{STR}_p\) &
\(\boldsymbol{\pi}^{FULL}_c\) &
\(\boldsymbol{\pi}^{STR}_c\) &
\(\boldsymbol{\pi}^{HSR}\) &
\(\boldsymbol{\pi}^{RND}\) &
\textit{\(\boldsymbol{\pi}^{MKT}\)} \\
\midrule
\multicolumn{8}{c}{\scriptsize \textit{Signal-to-noise ratio}} \\
\midrule
10 & 0.7782 & 0.7771 & 0.6277 & 0.6334 & 0.6471 & 0.7764 & \textit{0.8186} \\
20 & 0.8395 & 0.8391 & 0.7255 & 0.7242 & 0.7041 & 0.8287 & \textit{0.8186} \\
30 & 0.8547 & 0.8169 & 0.7512 & 0.7526 & 0.7368 & 0.8021 & \textit{0.8186} \\
40 & 0.8504 & 0.7907 & 0.7713 & 0.7684 & 0.7569 & 0.8484 & \textit{0.8186} \\
\midrule
\multicolumn{8}{c}{\scriptsize \textit{Average Return}} \\
\midrule
10 & 0.0771 & \textbf{0.0832} & 0.0642 & 0.0648 & 0.0637 & 0.0768 & \textit{0.0677} \\
20 & 0.0753 & \textbf{0.0798} & 0.0694 & 0.0692 & 0.0647 & 0.0651 & \textit{0.0677} \\
30 & 0.0719 & \textbf{0.0728} & 0.0693 & 0.0688 & 0.0664 & 0.0649 & \textit{0.0677} \\
40 & 0.0719 & \textbf{0.0728} & 0.0693 & 0.0688 & 0.0664 & 0.0649 & \textit{0.0677} \\
\midrule
\multicolumn{8}{c}{\scriptsize \textit{Volatility}} \\
\midrule
10 & 0.0990 & 0.1070 & 0.1023 & 0.1023 & 0.0988 & 0.0984 & \textit{0.0827} \\
20 & 0.0897 & 0.0951 & 0.0957 & 0.0956 & 0.0856 & 0.0918 & \textit{0.0827} \\
30 & 0.0881 & 0.0891 & 0.0914 & 0.0913 & 0.0828 & 0.0890 & \textit{0.0827} \\
40 & 0.0845 & 0.0921 & 0.0899 & 0.0895 & 0.0802 & 0.0877 & \textit{0.0827} \\
\bottomrule
\end{tabular*}
\end{table}

%\section{S \& P 500}










==> intro.tex <==

\begin{abstract}
Empirical correlation matrices estimated from financial return time series are contaminated by substantial statistical noise arising from finite sample size, obscuring the genuine interaction structure among assets. We apply spectral theory to decompose the empirical correlation matrix into a structured component associated with eigenvalues exceeding the Marchenko–Pastur bounds and a random component consistent with statistical noise. Using daily returns from three equity markets (NIFTY 200, NIFTY 500, and S\&P 500) spanning 2010 to 2022, we show that the structured component, constructed from only 10 to 16 eigenmodes, reproduces the principal statistical properties of the full correlation matrix while eliminating the majority of noise dominated eigenmodes. We then construct financial networks from the full, structured, and random correlation matrices and characterize their core-periphery organization using a Markov chain based method. The structured network exhibits significantly stronger and more stable core periphery organization than full or random networks. This observation is supported by degree preserving randomization tests together with Kolmogorov Smirnov and Wasserstein distance analyzes, which demonstrate a clear statistical separation between the structured and random components. We further show that the structured networks exhibit pronounced scale free degree distributions in the Indian markets, whereas the random networks do not, indicating that heterogeneous network topology emerges from genuine economic interactions rather than statistical noise. As a practical application, portfolios constructed from peripheral assets identified in the denoised network consistently achieve superior risk adjusted performance compared with portfolios based on the full correlation matrix and standard benchmark strategies. The robustness of these results is confirmed through Monte Carlo subsampling experiments. These findings demonstrate that spectral based denoising provides a general framework for recovering meaningful structural organization from noisy correlation networks, with financial portfolio construction representing one example of its broader applicability.
\end{abstract}

\maketitle

%\onecolumngrid


%\textbf{Financial markets are complex adaptive systems whose collective behavior emerges from intricate interactions among a large number of assets. However, empirical correlation matrices are often contaminated by statistical noise, making it difficult to distinguish a meaningful market structure from random fluctuations. In this work, we develop a network-guided portfolio optimization framework based on denoised correlation matrices obtained via spectral filtering. By isolating statistically significant collective modes and suppressing noise-dominated components, we construct financial networks that reveal the underlying interaction architecture of the market. Analysis of NIFTY 200, NIFTY 500, and S\&P 500 stocks demonstrates that portfolios built from the filtered network structure consistently achieve superior risk-adjusted performance compared to portfolios based on unfiltered correlations and conventional allocation benchmarks. The denoised networks also exhibit stable and statistically significant core–periphery organization over time, indicating that the extracted structures capture persistent features of market dynamics. These findings highlight the value of combining spectral theory and network science to uncover hidden organization in financial systems and to improve portfolio construction under uncertainty.}


\maketitle

\section{Introduction}
Complex systems composed of many interacting units are ubiquitous, span biological, technological, and social domains, and are frequently characterized by pairwise correlations observed between their constituent variables \cite{mantegna1999hierarchical, plerou2001collective}. A central obstacle to extracting genuine interaction structure from such systems is that empirical correlation matrices, estimated from finite time series, are inherently contaminated by statistical noise. When the number of observed variables is comparable to the length of the available time series, a regime routinely encountered in high-dimensional real-world data---a substantial fraction of the eigenspectrum of the empirical correlation matrix is indistinguishable from that of a purely random matrix \cite{Laloux1999noise, Plerou1999universal}. Distinguishing the small subset of eigenmodes that encode genuine collective structure from the majority that reflect sampling noise is therefore a prerequisite for any reliable downstream analysis of network topology, community organization, or predictive modeling built upon such correlations.

Financial markets provide a particularly well-studied and data-rich setting in which to address this problem. Stock return correlations are shaped by a mixture of genuine collective dynamics---driven by common macroeconomic factors, sectoral co-movement, and firm-level interdependence---and substantial estimation noise arising from finite sample size \cite{Plerou2001collective, jiang2014structure}. Portfolio optimization, which relies directly on accurate estimates of the covariance structure among assets, is especially sensitive to this contamination: classical mean--variance frameworks \cite{Markowitz1952,markowitz2000mean}, higher-moment extensions \cite{samuelson1970fundamental}, mean absolute deviation approaches \cite{konno1991mean,konno2005mean}, and downside-risk formulations \cite{nawrocki1992characteristics} all presuppose that the estimated correlation structure reflects genuine asset interdependence rather than noise, and their performance degrades accordingly when this assumption fails. This makes financial markets an ideal empirical setting for testing whether principled noise-filtering of correlation matrices can recover interpretable, economically meaningful structure---and, in turn, whether that structure has practical consequences for a canonical downstream task such as portfolio construction.



Recent advances have explored data-driven and heuristic approaches, including reinforcement learning and evolutionary optimization techniques, to address these limitations \cite{moody2001learning,aboussalah2020continuous,yusoff2011overview,reyes2006multi}. While flexible, these methods often suffer from limited interpretability, sensitivity to hyperparameters, and substantial computational costs. This has motivated increasing interest in network-based approaches, which aim to extract stable structural information from financial markets by representing assets as interconnected systems.

A central challenge in this context is that empirical correlation matrices are inherently noisy due to finite sample effects. To mitigate this issue, prior studies have analyzed the statistical properties of empirical correlation matrices through their spectral decomposition, noting that the bulk of eigenvalues can be well approximated by the Marchenko--Pastur distribution expected for purely random correlations \cite{plerou1999universal,laloux1999noise}. Specifically, eigenvalues within the Marchenko--Pastur bounds are consistent with random noise, whereas significant deviations correspond to genuine market structure, including collective and sectoral dynamics \cite{plerou2001collective,jiang2014structure}. While prior studies~\cite{kim2005systematic, pawanesh2025exploring} often focus on isolating the dominant market mode or a small number of sectoral components, it remains unclear how the full set of statistically significant eigenmodes can be leveraged for portfolio construction, particularly in conjunction with higher-order network structures.

In parallel, network representations of financial markets have provided valuable insights into systemic risk and market organization \cite{pozzi2013spread,ansari2025novel}. Beyond local connectivity measures, recent work highlights the importance of mesoscale structures, especially core--periphery (CP) organization~\cite{borgatti2000models, ansari2025uncovering, rombach2017core} in capturing the hierarchical structure of financial systems \cite{ansari2025novel, lee2014density}. Economically, core assets tend to be strongly interconnected and highly exposed to common market factors, whereas peripheral assets exhibit weaker correlations and greater idiosyncratic behavior. This suggests that peripheral assets may offer enhanced diversification benefits, although their systematic exploitation in portfolio design remains underexplored.

Against this backdrop, a key gap in the literature is the lack of an integrated framework that combines statistically grounded correlation denoising with mesoscale network structure for portfolio optimization. Existing studies typically treat these components in isolation, leaving unclear how their interaction influences portfolio performance. This research paper addresses this limitation by developing a network-guided portfolio construction framework that integrates eigenvalue spectrum-based denoising with core-periphery network analysis. Specifically, we construct filtered correlation matrices by retaining all eigenmodes that lie beyond the Marchenko--Pastur bounds and use these denoised correlations to build financial networks. We then exploit the core--periphery structure to guide asset selection, with a particular focus on peripheral stocks that are less exposed to common risk factors and thus provide stronger diversification potential.

Our contributions are threefold. First, we propose a unified framework that systematically combines spectral filtering and mesoscale network analysis for portfolio construction. Second, we provide new empirical evidence that portfolios constructed from peripheral assets in denoised networks achieve improved risk-adjusted performance relative to standard benchmarks, including random, high Sharpe Ratio, and unfiltered-correlation portfolios. Third, we demonstrate the robustness of these results across multiple markets including NIFTY~200, NIFTY~500, and S\&P~500, and across different allocation schemes, highlighting the stability and practical relevance of the proposed approach. Our findings show that improved portfolio performance arises from the joint effect of removing noisy correlations and exploiting higher-order market structure. By providing an interpretable and computationally efficient framework, this study contributes to the growing literature on network-based portfolio optimization and offers practical insights for portfolio management in complex and noisy financial environments.

%The remainder of the paper is organized as follows. Section~2 describes the data and methodology, including correlation filtering and core--periphery detection. Section~3 presents the empirical results and robustness analysis. Section~4 concludes.



==> methods.tex <==


%\subsection{Planar Maximally Filtered Graph}

%Filtering techniques are essential for extracting the most representative and significant connections in a network, thereby simplifying its structure while retaining key information~\cite{pozzi2013spread,sharma2019mutual,ansari2025novel}. The Planar Maximally Filtered Graph (PMFG)~\cite{tumminello2005tool} provides a robust method for this purpose and is widely used in the literature. In this study, we adopt the PMFG approach to analyze correlation-based networks. The methodology for constructing a PMFG subgraph is outlined below.

%Let \(G\) denote a graph with vertex set \(V(G)\) containing \(N\) vertices. A graph \(G\) is \textit{planar} if it can be embedded in the plane such that no two edges intersect except at their endpoints. According to \textit{Kuratowski's theorem}~\cite{west2001introduction}, a finite graph is \textit{planar} if and only if it does not contain a subgraph homeomorphic to \(K_5\) (the complete graph on 5 vertices) or \(K_{3,3}\) (the complete 3-3 bipartite graph). A planar graph is called \textit{maximal planar} if adding any additional edge would violate planarity.

%The PMFG construction begins by sorting the elements of the upper triangular part of the adjacency matrix in descending order. Initially, the first six elements are selected, and the corresponding vertices and edges are included to form the initial PMFG. Subsequently, for each remaining element in the sorted list, the associated vertices and edges are tentatively added, and the planarity condition is tested using the \textit{Boyer–Myrvold planarity algorithm}~\cite{boyer2006simplified}. If planarity is preserved, the graph is updated to include the new edge. This iterative procedure continues until all elements of the sorted list have been considered. The resulting PMFG contains exactly \(3(N - 2)\) edges, forming a \textit{maximally filtered planar graph} that retains the most significant structural information from the original network.



\section{Methodology}

\subsection{Data description}

This study uses three datasets from the Indian National Stock Exchange (NSE) and the U.S. stock market, namely the NIFTY~200, NIFTY~500, and S\&P~500 indices. The datasets comprise daily closing prices of all constituent stocks from January~1,~2010, to December~31,~2022. To ensure data completeness, stocks with missing observations were excluded. This filtering resulted in refined datasets consisting of 140 stocks over 3{,}208 trading days for the NIFTY~200, 312 stocks over 3{,}204 trading days for the NIFTY~500, and 425 stocks over 3{,}271 trading days for the S\&P~500 index.

The daily logarithmic return for stock \(i\) at time \(t\) is defined as
\[
r_i(t) = \ln \left (\frac{p_i(t)} { p_i(t-1)}\right),
\]
where \(p_i(t)\) denotes the closing price of stock \(i\) on day \(t\).





Figure~\ref{fig:nifty} shows the NIFTY~200 index, the NIFTY~500 index, and the S\&P~500 index, providing an overview of the three stock markets. This datasets includes the COVID-19 pandemic period, which captures a global crisis phase. Incorporating this period allows us to examine portfolio behavior and risk dynamics under extreme market stress conditions.

%N = 140, T = 3208, N = 312, T = 3204, N = 425, T = 3271

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/figures/Index_Comparison_2010_2022.png}
    \caption{Time series plot of NIFTY 200, NIFTY 500 and S\&P 500 indices.}
    \label{fig:nifty}
\end{figure}



%\subsection{Correlation Matrix of Returns}

\subsection{Correlation matrix eigenvalue spectrum}

Let $r_i(t)$ denote the daily logarithmic return of the stock $i$, where $i = 1,2,\ldots,N$ and $N$ is the total number of stocks in the data set. The time index spans $t = 1,2,\ldots,T$, with $T$ denoting the total number of observations. Since different stocks exhibit varying levels of volatility ( measured by the standard deviation of their returns), we define the normalized return as
\begin{equation}
\tilde{r}_i(t) = \frac{r_i(t) - \langle r_i \rangle}{\sigma_i},
\end{equation}
where $\sigma_i = \sqrt{\langle r_i^2 \rangle - \langle r_i \rangle^2}$, is the standard deviation of $r_i(t)$, and $\langle \cdot \rangle$ denotes the time average over the observation period.


The cross-correlation matrix $C = [C_{ij}]$ is constructed from the normalized return series $\tilde{r}_i(t)$ as
\begin{equation}
C_{ij} = \left\langle \tilde{r}_i(t)\ \tilde{r}_j(t) \right\rangle
\end{equation}
%where $\langle \cdot \rangle$ denotes the time average over the observation period.

%Equivalently, in terms of the original return series $r_i(t)$, the correlation coefficient can be written as
%\begin{equation}
%C_{ij} = \frac{\langle r_i r_j \rangle - \langle r_i \rangle \langle r_j \rangle}{\sqrt{\langle r_i^2 \rangle - \langle r_i \rangle^2}\,
%\sqrt{\langle r_j^2 \rangle - \langle r_j \rangle^2}}.
%\end{equation}

The resulting matrix $C$ is real and symmetric, with diagonal elements $C_{ii}=1$, and all entries satisfying $-1 \leq C_{ij} \leq 1$.

%In the limit of a large number of variables $N$ and large sample size $T$, 
%and under the null hypothesis that the correlation matrix is random, 
%the eigenvalue distribution of $C$ can be approximated by the Marchenko–Pastur distribution. 
%To quantify this, we compare the spectral properties of the empirical correlation matrix $C$ 
%with those of a random correlation (Wishart) matrix~\cite{baker1998random}. 




\begin{figure}[htbp]
    \centering

    % Top row: two plots side by side
    \begin{subfigure}[b]{0.39\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/eigen_density_Nifty200_2010_22.png}
        \caption{}
        \label{fig:nifty200}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.39\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/eigen_density_Nifty500_2010_22.png}
        \caption{}
        \label{fig:nifty500}
    \end{subfigure}

    \vspace{0.6cm} % vertical space between rows

    % Bottom row: single centered plot
    \begin{subfigure}[b]{0.39\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/eigen_density_SP00_2010_22.png} % fixed filename
        \caption{}
        \label{fig:sp500}
    \end{subfigure}

\caption{Eigenmode plots for (a) NIFTY~200, (b) NIFTY~500, and (c) S\&P~500 over the period from January~1,~2010, to December~31,~2022. Here, $\lambda_{-}$ and $\lambda_{+}$ denote the Marčenko--Pastur (MP) bounds, and $\lambda_{m}$ represents the largest eigenvalue of the empirical correlation matrix.}

    \label{fig:eigen_modes_plot}
\end{figure}








\begin{table}[htbp]
\centering
\caption{Spectral properties of empirical correlation matrix. 
$\lambda_{-}$ and $\lambda_{+}$ denote the theoretical Marčenko--Pastur (MP) bounds and $\lambda_{\max}$ is the largest eigenvalue of the empirical correlation matrix. 
Percentages indicate the proportion of empirical eigenvalues ($\hat{\lambda}$) lying below $\lambda_{-}$, within the MP bulk $(\lambda_{-}<\hat{\lambda}<\lambda_{+})$, and above $\lambda_{+}$.}
\label{tab:rmt_spectral}
\resizebox{\textwidth}{!}{
\begin{tabular}{l c c c c c c}
\hline
Dataset & $\lambda_{-}$ & $\lambda_{+}$ & $\lambda_{\max}$ & 
$\hat{\lambda}<\lambda_{-}$ (\%) & 
$\lambda_{-}<\hat{\lambda}<\lambda_{+}$ (\%) & 
$\hat{\lambda}>\lambda_{+}$ (\%) \\
\hline

NIFTY 200 & 0.626 & 1.461 & 35.87 & 46.43 & 46.43 & 7.14 \\

NIFTY 500 & 0.473 & 1.722 & 68.62 & 25.00 & 71.15 & 3.85 \\

S\&P 500 & 0.409 & 1.851 & 172.15 & 57.65 & 38.59 & 3.76 \\

\hline
\end{tabular}
}
\end{table}



%The statistical properties of empirical correlation matrices have been extensively studied in the literature~\cite{gopikrishnan2001quantifying, jiang2014structure, macmahon2015community, purqon2021community}. 

If the $N$ return time series of length $T$ consists of independent and identically distributed Gaussian random variables with zero mean and unit variance, then the resulting random correlation matrix follows a Wishart distribution.

In the asymptotic limit $N \to \infty$ and $T \to \infty$ with the ratio 

\[
Q = \frac{T}{N} \geq 1
\]

held fixed, the probability density function of the eigenvalues $\lambda$ of the random correlation matrix converges to the Marchenko--Pastur distribution~\cite{pastur2011eigenvalue}, given by

\begin{equation}
P_{\text{rm}}(\lambda) =
\begin{cases}
\displaystyle
\frac{Q}{2\pi \lambda} 
\sqrt{(\lambda_{+} - \lambda)(\lambda - \lambda_{-})}, 
& \text{if } \lambda_{-} \leq \lambda \leq \lambda_{+}, \\[10pt]
0, & \text{otherwise},
\end{cases}
\end{equation}

where $\lambda_{-}$ and $\lambda_{+}$ denote the lower and upper bounds of the eigenvalue spectrum, defined as

\begin{equation}
\lambda_{-} = \left(1 - \frac{1}{\sqrt{Q}}\right)^2, 
\qquad 
\lambda_{+} = \left(1 + \frac{1}{\sqrt{Q}}\right)^2.
\end{equation}

The cross-correlation matrix \(C\) can be decomposed into a set of orthogonal eigenmodes as
\[
C_{ij} = \sum_{\gamma=1}^{N} C_{ij}^{\gamma},
\]
where
\[
C_{ij}^{\gamma} = \lambda_{\gamma} u_i^{\gamma} u_j^{\gamma}.
\]
Here, \(\lambda_{\gamma}\) denotes the \(\gamma\)-th eigenvalue of \(C\), and \(u_i^{\gamma}\) represents the \(i\)-th component of the corresponding eigenvector.

We decomposed the empirical cross-correlation matrix into two components—namely, the structured mode, and the random mode as follows. The \emph{structured mode} $C^{\mathrm{STR}}$ is given by $C^{\mathrm{STR}}_{ij} = \sum_{\gamma=1}^{k} C^{\gamma}_{ij}$, where \(k\) denotes the number of eigenvalues lying above the upper bound of the Marchenko--Pastur interval \([\lambda_{-}, \lambda_{+}]\), capturing the structured (non-random) correlations. The \emph{random mode} $C^{\mathrm{RND}}$ is defined as $C^{\mathrm{RND}}_{ij} = \sum_{\gamma=k+1}^{N} C^{\gamma}_{ij}$, which represents noise-driven correlations.

Throughout the 13-year dataset, we find that for the NIFTY~200 index, the 10 largest eigenvalues fall within the structured mode, while for the NIFTY~500 and S\&P~500 indices, 12 and 16 eigenvalues are identified, respectively. Table~\ref{tab:rmt_spectral} shows the spectral properties of empirical correlation matrix. Figure~\ref{fig:eigen_modes_plot} presents the eigenmode plots for the NIFTY~200, NIFTY~500, and S\&P~500. Subsequently, networks are constructed from the full cross-correlation matrix $C^{\mathrm{FULL}}$, the structured-mode matrix $C^{\mathrm{STR}}$, and the random-mode matrix $C^{\mathrm{RND}}$. Figure~\ref{fig:corr_distribution} shows the probability density functions of the elements of the correlation matrices for the NIFTY~200, NIFTY~500, and S\&P~500. The distributions corresponding to the full and structured-mode correlation matrices are in close agreement, highlighting that the structured-mode matrix constructed using only a few eigenvalues lying beyond the Marchenko--Pastur bounds captures the dominant correlation structure of the market. 



\begin{figure}[htbp]
    \centering
    % Top row: two plots side by side
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/figures/corr_distribution_FULL_STR_RND_NIFTY200.png}
        \caption{}
        \label{fig:nifty200}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/figures/corr_distribution_FULL_STR_RND_NIFTY500.png}
        \caption{}
        \label{fig:nifty500}
    \end{subfigure}

    \vspace{0.6cm} % vertical space between rows

    % Bottom row: single centered plot
    \begin{subfigure}[b]{0.42\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/figures/corr_distribution_FULL_STR_RND_SP500.png} % fixed filename
        \caption{}
        \label{fig:sp500}
    \end{subfigure}

\caption{Kernel density estimates of the empirical distribution of pairwise correlation coefficients ($C_{ij}$) for (a) NIFTY 200, (b) NIFTY 500, and (c) S\&P 500 over the period January 1, 2010 to December 31, 2022.}    
    \label{fig:corr_distribution}
\end{figure}


\subsection{Core-periphery structure of networks}

Network science has devoted considerable effort to uncovering the core–periphery structure, a key mesoscale organization pattern observed in diverse real-world networks. Detecting core–periphery structure in networks is crucial for uncovering hierarchical relationships and understanding the organization of complex systems~\cite{borgatti2000models,boyd2006computing,rombach2017core}. 

Our study employs the iterative algorithm to extract the \textit{core–periphery profile} of the network as proposed in~\cite{rossa2013profiling}. This algorithm is grounded in Markov chain theory and provides a probabilistic measure of persistence within the core and periphery subsets. It offers a rigorous and comprehensive framework for analyzing core–periphery structures across a wide range of network types. In this formulation, the vertices of the network correspond to the states of a Markov chain, and the transition probability matrix \( (p_{ij}) \) is defined as $p_{ij} = \frac{a_{ij}}{\displaystyle\sum_{h \in V(G)} a_{ih}}$, where \( a_{ij} \) denotes the weight of the edge between vertices \( i \) and \( j \), with \( i,j,h \in V(G) \). 

%We assume that the network is undirected, i.e., \( a_{ij} = a_{ji} \), and that all vertices have positive strength (\(C_D(i) > 0\)), ensuring the corresponding Markov chain is ergodic. This transformation guarantees non-negative edge weights, allowing for a valid probabilistic interpretation within the Markovian framework.

Let \(S \subseteq G\) denote a subgraph of \(G\), with vertex set \(V(S) \subseteq V(G)\). The \textit{persistence probability} \(\gamma_{\strut S} \) quantifies the internal cohesiveness of \(S\) and is defined as
\[
\gamma_{\strut S}  =  \frac{\displaystyle\sum_{i,j \in V(S)} \pi_i p_{ij}}{\displaystyle\sum_{i \in V(S)} \pi_i},
\]
where \(\pi_i > 0\) is the stationary probability of being at vertex \(i\)~\cite{meyer2023matrix}, given by
\[
\pi_i = \frac{C_D(i)}{\displaystyle\sum_{j \in V(G)} C_D(j)} \quad \text{with} \quad 
C_D(i) = \sum_{h \in V(G)} a_{ih},
\]
and \(C_D(i)\) denotes the weighted degree (strength) of vertex \(i\). Using this formulation, \(\gamma_{\strut S} \) simplifies to
\begin{equation}
\label{eq:community_connectivity}
\gamma_{\strut S}  = \frac{\displaystyle \sum_{i,j \in V(S)} a_{ij}}{\displaystyle\sum_{i \in V(S),\, j \in V(G)} a_{ij}},
\end{equation}
which provides a computationally efficient and interpretable measure of subgraph cohesiveness.

The coreness values are determined iteratively. The process begins with the vertex having the smallest weighted degree, denoted as \( S_1 = \{1\} \), for which \( \gamma_1 \equiv \gamma_{S_1} = 0 \).  
For the next iteration, consider all subsets \( S_2^{(j)} = S_1 \cup \{j\} \) for \( 2 \le j \le N \), and compute \( \gamma_{S_2^{(j)}} \) for each.  
The subset \( S_2 \) corresponding to the minimum persistence probability \( \gamma_{S_2^{(k)}} \) is selected, and \( \gamma_2 \equiv \gamma_{S_2} \) is assigned as the coreness of vertex \( k \). This ensures \( \gamma_1 \le \gamma_2 \). The process continues iteratively: \( S_3 \) is formed from \( S_2 \) by adding one vertex at a time such that \( \gamma_3 \) is minimized, ensuring
\[
\gamma_1 \le \gamma_2 \le \gamma_3 \le \cdots \le \gamma_N.
\]

Thus, each vertex receives a coreness value corresponding to its inclusion in the sequence of subsets that minimizes the persistence probability. In Figure~\ref{fig:adjacency_plot}, we plot the permuted adjacency matrices from the full ($C^{\mathrm{FULL}}$), structured ($C^{\mathrm{STR}}$), and random ($C^{\mathrm{RND}}$) mode matrices for the NIFTY 200, NIFTY 500, and S&P 500 over the entire 13-year period. The matrices are permuted by ordering rows and columns in decreasing order of coreness values. A clear core--periphery block structure is observed for the full and structured-mode networks; however, no such structure is evident for the random-mode network.



\begin{figure}[htbp]
    \centering

    % NIFTY 200
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/figures/adjacency_CP_Nifty200.png}
        \caption{NIFTY 200}
        \label{fig:adjacency_nifty200}
    \end{subfigure}
    
    \vspace{0.3cm} % vertical space
    
    % NIFTY 500
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/adjacency_CP_Nifty500.png}
        \caption{NIFTY 500}
        \label{fig:adjacency_nifty500}
    \end{subfigure}

    \vspace{0.3cm} % vertical space
    
    % S&P 500
    \begin{subfigure}[b]{1.0\textwidth}
        \centering
        \includegraphics[width=1.0\textwidth]{figures/figures/adjacency_CP_SP500.png}
        \caption{S\&P 500}
        \label{fig:adjacency_sp500}
    \end{subfigure}

    \caption{Permuted adjacency matrix plots of NIFTY 200, NIFTY 500, and S\&P 500 indices.}
    \label{fig:adjacency_plot}
\end{figure}


\subsection{Portfolio weight allocation and performance evaluation}

Markowitz mean--variance portfolio theory~\cite{Markowitz1952} provides a cornerstone of modern portfolio selection by formalizing the trade-off between expected return and risk. Within this framework, portfolio optimization can be naturally cast in terms of the Sharpe ratio, which quantifies the excess return achieved per unit of risk and is therefore widely adopted as a measure of risk-adjusted performance~\cite{cornuejols2005optimization}.  

In this study, we construct portfolios by maximizing the Sharpe ratio under standard budget and long-only constraints. Let $\mathbf{w} = (w_1,\dots,w_N)^\top$ denote the vector of portfolio weights assigned to the $N$ assets, $\boldsymbol{\mu}$ the vector of expected asset returns, and $\mathbf{\Sigma}$ the corresponding covariance matrix, estimated from the empirical correlation matrix. The optimal portfolio weights are obtained by solving the following optimization problem:
\begin{equation}
\max_{\mathbf{w}} \;
\frac{\boldsymbol{\mu}^{\top}\mathbf{w} - r_f}
{\sqrt{\mathbf{w}^{\top}\mathbf{\Sigma}\mathbf{w}}}
\quad \text{s.t.} \quad
\sum_{i=1}^{N} w_i = 1 , 
\quad 0 \le w_i \le 1 \ ; \forall i .
\end{equation}

Here, $r_f$ denotes the risk-free rate, which is set to zero throughout this work without loss of generality. This formulation ensures full capital allocation and excludes short-selling, reflecting realistic investment constraints.

To evaluate portfolio performance, let $\hat{S}_{t,i}$ denote the price of asset $i$ at time $t$. For a portfolio consisting of selected assets $m$, the logarithmic return of the asset $i$ over a holding period $T$ is defined as
\begin{equation}
r_{t+T,i} = \ln \left( \frac{\hat{S}_{t+T,i}}{\hat{S}_{t,i}} \right),
\end{equation}
and the corresponding portfolio return is given by
\begin{equation}
r_{t+T,m} = \sum_{i=1}^{m} w_i \, r_{t+T,i}.
\end{equation}

For each holding period $T$, we compute the time-averaged portfolio return $\bar{r}_{t+T,m}$ and its standard deviation $\sigma_{T,m}$ over the full observation window. The portfolio signal-to-noise ratio is then defined as
\begin{equation}
SR_{T,m} = \frac{\bar{r}_{t+T,m}}{\sigma_{T,m}}.
\end{equation}

From an investment perspective, portfolios with a higher signal-to-noise ratio are preferred as they deliver superior risk-adjusted performance. Consequently, comparing $SR_{T,m}$ across portfolios constructed using different correlation estimators provides a robust and economically meaningful basis to assessing the impact of denoising on portfolio efficiency.

==> results.tex <==


\section{Results \& discussion}


\subsection{Background and investment strategies}

We used daily log-returns of 140 stocks from the NIFTY 200, 314 stocks from the NIFTY 500 (National Stock Exchange of India), and 425 stocks from the S\&P 500 (U.S. equity market) over the period January 2010 to December 2022. This sample includes major market disruptions, such as the COVID-19 crash of 2020, ensuring a realistic and volatile market environment (see Fig.~\ref{fig:nifty}). To construct portfolios, we employ one day rolling windows of length 500 trading days. For each window, we estimate the empirical correlation matrix \(C^{\mathrm{FULL}}\) and its denoised counterpart \(C^{\mathrm{STR}}\), obtained by retaining statistically significant eigenmodes. The financial networks are then constructed from these matrices and their core--periphery (CP) structures are identified using the Markov chain–based random walk method \cite{rossa2013profiling}. The top-\(M\) core or periphery stocks are selected for portfolio construction, and out-of-sample performance is evaluated over the subsequent 125 trading days.

From a practical perspective, constructing portfolios from a large universe of assets is often associated with high transaction costs and operational complexity. Therefore, our framework focuses on selecting a relatively small subset of informative stocks. To evaluate scalability and diversification effects, we consider portfolio sizes \(M = 10, 20, 30, 40\), allowing us to examine the trade-off between diversification benefits and portfolio manageability. We consider the following portfolio strategies. Let \(\boldsymbol{\pi}^{(s)}_x\) denote a portfolio constructed from network type \(s \in \{\mathrm{FULL}, \mathrm{STR}\}\), where \(x \in \{c, p\}\) indicates whether assets are selected from the core or the periphery. Thus, \(\boldsymbol{\pi}^{(s)}_c\) and \(\boldsymbol{\pi}^{(s)}_p\) represent core- and periphery-based portfolios, respectively.

In addition to CP-based strategies, we include two benchmark portfolios. First, the \emph{highest Sharpe ratio} strategy, denoted by \(\boldsymbol{\pi}^{\mathrm{HSR}}\), selects the top-\(M\) stocks with the highest in-sample Sharpe ratios, representing a return–risk optimal stock-picking benchmark without network information. Second, the \emph{random selection} strategy, denoted by \(\boldsymbol{\pi}^{\mathrm{RND}}\), selects \(M\) stocks uniformly at random, serving as a baseline. Finally, we consider the \emph{market portfolio}, denoted by \(\boldsymbol{\pi}^{\mathrm{MKT}}\), which includes all available stocks in the respective index (140 for NIFTY 200, 314 for NIFTY 500, and 425 for S\&P 500), with weights assigned either uniformly or via Markowitz optimization. This portfolio serves as a broad benchmark for comparison.

\subsection{Comparative study on portfolio performance}

This section evaluates the out-of-sample performance of portfolio strategies derived from the core--periphery structure of correlation networks across three equity universes: NIFTY~200, NIFTY~500, and S\&P~500. Results are reported for portfolio sizes $M=\{10,20,30,40\}$ under both equal-weighted and Markowitz-weighted schemes. We compare portfolios constructed from core and peripheral stocks of both full and structured correlation networks against benchmark strategies, including the highest Sharpe ratio portfolio ($\boldsymbol{\pi}^{HSR}$), random selection ($\boldsymbol{\pi}^{RND}$), and the market portfolio ($\boldsymbol{\pi}^{MKT}$).

Across the NIFTY~200 and NIFTY~500 universes, portfolios constructed from peripheral stocks of the structured correlation network ($\boldsymbol{\pi}^{STR}_p$) consistently deliver the strongest risk-adjusted performance. As shown in Tables~\ref{tab:nifty_200_uniform} and \ref{tab:nifty_500_uniform}, their signal-to-noise ratios increase with portfolio size, indicating that moderate diversification within the periphery enhances portfolio efficiency. For instance, in the NIFTY~200 universe, the signal-to-noise ratio rises from approximately $0.6$ for $M=10$ to $0.8$ for $M=40$, substantially exceeding both the market portfolio and the $\boldsymbol{\pi}^{HSR}$ benchmark. This superior performance is driven by a combination of higher average returns and lower volatility relative to competing strategies. In contrast, core-based portfolios ($\boldsymbol{\pi}^{FULL}_c$ and $\boldsymbol{\pi}^{STR}_c$) consistently underperform across portfolio sizes. Their lower signal-to-noise ratios reflect limited diversification benefits, as core stocks exhibit strong co-movement with the broader market. The S\&P~500 universe exhibits a more muted pattern. While peripheral portfolios remain competitive, their advantage over the market portfolio is less pronounced (Table~\ref{tab:sp_500_uniform}). This is consistent with the higher level of inherent diversification in the U.S. market, where the benchmark portfolio already captures a broad range of risk factors.


Applying Markowitz optimization improves signal-to-noise ratios across all strategies by explicitly accounting for the return--risk trade-off. In the NIFTY~200 universe, structured periphery portfolios continue to perform strongly, with signal-to-noise ratios increasing from $0.69$ for $M=10$ to $1.21$ for $M=40$. Notably, these gains are achieved using only a subset of available assets, highlighting the efficiency of network-based selection. A similar pattern is observed in the NIFTY~500 universe, where structured periphery portfolios exhibit stable and competitive performance as portfolio size increases. Although the market portfolio attains the highest signal-to-noise ratio overall, the network-based portfolios remain close while requiring significantly fewer assets. In the S\&P~500 universe, peripheral portfolios continue to deliver competitive outcomes, though consistently outperforming the market benchmark remains challenging.


These findings reveal a systematic link between network topology and portfolio diversification. Core stocks, by construction, are highly interconnected and therefore strongly exposed to common market factors, limiting their diversification potential. Peripheral stocks, on the contrary, exhibit weaker correlations and lower systemic exposure, allowing them to contribute more effectively to risk reduction. From a practical point of view, the proposed framework enables the construction of efficient portfolios using a relatively small subset of assets. This has important implications for implementation, including reduced transaction costs, improved manageability, and lower computational complexity. Finally, the results demonstrate that the combination of correlation denoising with the mesoscale network structure provides a robust and economically meaningful enhancement to traditional portfolio construction methods.


  
\subsection{Monte Carlo--based robustness analysis}

To assess the robustness and statistical significance of the proposed strategy, we employ a Monte Carlo--based subsampling framework. Let \( B^{(k)} \in \mathbb{R}^{T \times W} \) denote the matrix of out-of-sample portfolio returns corresponding to strategy \( k \), where \( T = 250 \) is the investment horizon and \( W \) is the number of rolling windows. The strategies under consideration are
\[
\boldsymbol{\pi}^{FULL}_p,\;
\boldsymbol{\pi}^{STR}_p,\;
\boldsymbol{\pi}^{FULL}_c,\;
\boldsymbol{\pi}^{STR}_c,\;
\boldsymbol{\pi}^{HSR},\;
\boldsymbol{\pi}^{RND},\;
\boldsymbol{\pi}^{MKT},
\]
where \( \boldsymbol{\pi}^{STR}_p \) represents the proposed strategy.

At each iteration \( m = 1, \ldots, M \) (with \( M = 1000 \)), we randomly select a subset of \( n = 500 \) rolling windows without replacement:
\[
\mathcal{I}_m \subset \{1,\ldots,W\},
\qquad
|\mathcal{I}_m| = 500.
\]

For each strategy \( k \), the corresponding returns are pooled across the selected windows to form
\[
\mathcal{R}_m^{(k)}
=
\left\{
B^{(k)}_{t,i}
:
i \in \mathcal{I}_m,\;
t = 1,\ldots,T
\right\}.
\]

The annualized Sharpe ratio for strategy \( k \) in iteration \( m \) is computed as
\[
S_m^{(k)}
=
\frac{\mu_m^{(k)}}{\sigma_m^{(k)}}\sqrt{252},
\]
where \( \mu_m^{(k)} \) and \( \sigma_m^{(k)} \) denote the sample mean and standard deviation of \( \mathcal{R}_m^{(k)} \), respectively. The risk-free rate is assumed to be zero.

To evaluate whether the superior performance of the proposed strategy is statistically significant, we compare its Sharpe ratio with that of each benchmark across all Monte Carlo replications. Let
\begin{equation}
\Delta_m^{(j)}
=
S_m^{(\pi_p^{STR})}
-
S_m^{(j)},
\qquad
m = 1,\ldots,M,
\end{equation}
denote the Sharpe ratio difference between the proposed strategy and benchmark \( j \) in replication \( m \).

Since the distribution of Sharpe ratio differences may deviate from normality, we employ the nonparametric Wilcoxon signed-rank test. Specifically, we test
\[
H_0:\operatorname{median}\!\left(\Delta_m^{(j)}\right)=0
\]
against the one-sided alternative
\[
H_1:\operatorname{median}\!\left(\Delta_m^{(j)}\right)>0.
\]

Rejection of the null hypothesis indicates that the proposed strategy delivers significantly higher risk-adjusted performance than the corresponding benchmark.

In addition, we report the win proportion
\begin{equation}
\hat{p}^{(j)}
=
\frac{1}{M}
\sum_{m=1}^{M}
\mathbf{1}
\!\left(
S_m^{(\pi_p^{STR})}
>
S_m^{(j)}
\right),
\end{equation}
which measures the fraction of Monte Carlo replications in which the proposed strategy achieves a higher Sharpe ratio than the benchmark \( j \). Together, \( \hat{p}^{(j)} \) and the Wilcoxon p-value provide complementary evidence on the consistency and statistical significance of the observed performance.

 
\begin{table}[htbp]
\centering
\footnotesize
\caption{Monte Carlo-based robustness analysis of the proposed strategy $\pi^{STR}_p$ against benchmark strategies. Each entry reports the win proportion $\hat{p}$ and the corresponding Wilcoxon signed-rank test p-value. Results are shown for equal-weighted ($\boldsymbol{w}^{EW}$) and Markowitz-weighted ($\boldsymbol{w}^{MW}$) portfolios across portfolio sizes $M=\{10,20,30,40\}$ using NIFTY 200 stocks.}
\label{tab:mc_robustness_nifty200}

\begin{tabular*}{0.95\textwidth}{@{\extracolsep{\fill}} l l c c c c c c}
\toprule
\textbf{M} & \textbf{Weight} &
$\boldsymbol{\pi}^{FULL}_p$ &
$\boldsymbol{\pi}^{FULL}_c$ &
$\boldsymbol{\pi}^{STR}_c$ &
$\boldsymbol{\pi}^{HSR}$ &
$\boldsymbol{\pi}^{RND}$ &
$\boldsymbol{\pi}^{MKT}$ \\
\midrule

\multirow{2}{*}{10}
& $\boldsymbol{w}^{EW}$
& \makecell{0.96\\($p<10^{-160}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\


\cmidrule(lr){2-8}

& $\boldsymbol{w}^{MW}$
& \makecell{0.00\\($p=1.00$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.94\\($p<10^{-155}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.00\\($p=1.00$)} \\
\midrule

\multirow{2}{*}{20}
& $\boldsymbol{w}^{EW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\

\cmidrule(lr){2-8}

& $\boldsymbol{w}^{MW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.00\\($p=1.00$)} \\
\midrule

\multirow{2}{*}{30}
& $\boldsymbol{w}^{EW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\

\cmidrule(lr){2-8}

& $\boldsymbol{w}^{MW}$
& \makecell{0.00\\($p=1.00$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.98\\($p<10^{-163}$)}
& \makecell{0.00\\($p=1.00$)} \\
\midrule

\multirow{2}{*}{40}
& $\boldsymbol{w}^{EW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\

\cmidrule(lr){2-8}

& $\boldsymbol{w}^{MW}$
& \makecell{0.34\\($p=1.00$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.19\\($p=1.00$)}
& \makecell{0.00\\($p=1.00$)} \\
\bottomrule
\end{tabular*}
\end{table}
   


\begin{table}[htbp]
\centering
\footnotesize
\caption{Monte Carlo-based robustness analysis of the proposed strategy $\pi^{STR}_p$ against benchmark strategies. Each entry reports the win proportion $\hat{p}$ and the corresponding Wilcoxon signed-rank test p-value. Results are shown for equal-weighted ($\boldsymbol{w}^{EW}$) and Markowitz-weighted ($\boldsymbol{w}^{MW}$) portfolios across portfolio sizes $M=\{10,20,30,40\}$ using NIFTY 500 stocks.}
\label{tab:mc_robustness_nifty500}

\begin{tabular*}{0.95\textwidth}{@{\extracolsep{\fill}} l l c c c c c c}
\toprule
\textbf{M} & \textbf{Weight} &
$\boldsymbol{\pi}^{FULL}_p$ &
$\boldsymbol{\pi}^{FULL}_c$ &
$\boldsymbol{\pi}^{STR}_c$ &
$\boldsymbol{\pi}^{HSR}$ &
$\boldsymbol{\pi}^{RND}$ &
$\boldsymbol{\pi}^{MKT}$ \\
\midrule

\multirow{2}{*}{10}
& $\boldsymbol{w}^{EW}$
& \makecell{0.03\\($p=1.00$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\
\cmidrule(lr){2-8}
& $\boldsymbol{w}^{MW}$
& \makecell{0.01\\($p=1.00$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.00\\($p=1.00$)} \\

\midrule

\multirow{2}{*}{20}
& $\boldsymbol{w}^{EW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\
\cmidrule(lr){2-8}
& $\boldsymbol{w}^{MW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.25\\($p=1.00$)} \\
\midrule

\multirow{2}{*}{30}
& $\boldsymbol{w}^{EW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\
\cmidrule(lr){2-8}
& $\boldsymbol{w}^{MW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.70\\($p<10^{-46}$)} \\

\midrule

\multirow{2}{*}{40}
& $\boldsymbol{w}^{EW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\
\cmidrule(lr){2-8}
& $\boldsymbol{w}^{MW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.97\\($p<10^{-161}$)} \\
\bottomrule
\end{tabular*}
\end{table}



\begin{table}[htbp]
\centering
\footnotesize

\caption{Monte Carlo-based robustness analysis of the proposed strategy $\pi^{STR}_p$ against benchmark strategies. Each entry reports the win proportion $\hat{p}$ and the corresponding Wilcoxon signed-rank test p-value. Results are shown for equal-weighted ($\boldsymbol{w}^{EW}$) and Markowitz-weighted ($\boldsymbol{w}^{MW}$) portfolios across portfolio sizes $M=\{10,20,30,40\}$ using S\&P 200 stocks.}

\label{tab:mc_robustness_sp500}

\begin{tabular*}{0.95\textwidth}{@{\extracolsep{\fill}} l l c c c c c c}
\toprule
\textbf{M} & \textbf{Weight} &
$\boldsymbol{\pi}^{FULL}_p$ &
$\boldsymbol{\pi}^{FULL}_c$ &
$\boldsymbol{\pi}^{STR}_c$ &
$\boldsymbol{\pi}^{HSR}$ &
$\boldsymbol{\pi}^{RND}$ &
$\boldsymbol{\pi}^{MKT}$ \\
\midrule

\multirow{2}{*}{10}
& $\boldsymbol{w}^{EW}$
& \makecell{0.62\\($p<10^{-18}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\
\cmidrule(lr){2-8}
& $\boldsymbol{w}^{MW}$
& \makecell{0.88\\($p<10^{-132}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.32\\($p=1.00$)} \\
\midrule

\multirow{2}{*}{20}
& $\boldsymbol{w}^{EW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\
\cmidrule(lr){2-8}
& $\boldsymbol{w}^{MW}$
& \makecell{0.98\\($p<10^{-163}$)}
& \makecell{0.89\\($p<10^{-138}$)}
& \makecell{0.85\\($p<10^{-123}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{0.94\\($p<10^{-154}$)}
& \makecell{0.40\\($p=1.00$)} \\
\midrule

\multirow{2}{*}{30}
& $\boldsymbol{w}^{EW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\
\cmidrule(lr){2-8}
& $\boldsymbol{w}^{MW}$
& \makecell{0.19\\($p=1.00$)}
& \makecell{0.79\\($p<10^{-94}$)}
& \makecell{0.82\\($p<10^{-108}$)}
& \makecell{1.00\\($p<10^{-164}$)}
& \makecell{0.00\\($p=1.00$)}
& \makecell{0.06\\($p=1.00$)} \\
\midrule

\multirow{2}{*}{40}
& $\boldsymbol{w}^{EW}$
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)}
& \makecell{1.00\\($p<10^{-165}$)} \\
\cmidrule(lr){2-8}
& $\boldsymbol{w}^{MW}$
& \makecell{0.86\\($p<10^{-126}$)}
& \makecell{0.13\\($p=1.00$)}
& \makecell{0.20\\($p=1.00$)}
& \makecell{0.92\\($p<10^{-152}$)}
& \makecell{0.09\\($p=1.00$)}
& \makecell{0.01\\($p=1.00$)} \\
\bottomrule
\end{tabular*}
\end{table}



This framework evaluates performance consistency across different subsets of market conditions rather than relying on a single realization. By repeatedly subsampling rolling windows, we obtain a distribution of relative performance outcomes that captures variability across market regimes. The empirical results, summarized in Tables~\ref{tab:mc_robustness_nifty200}--\ref{tab:mc_robustness_sp500}, show that the proposed strategy consistently outperforms competing strategies, as reflected by high win proportions $\hat{p}$ and statistically significant p-values from the Wilcoxon signed-rank test. In most comparisons, the win proportion $\hat{p}$ is close to unity, providing strong evidence against the null hypothesis of no dominance. This indicates that the observed performance improvements are not driven by a specific subset of rolling windows but persist across a wide range of sampled market conditions.

Across both NIFTY 200 and NIFTY 500 datasets, the proposed strategy demonstrates strong and statistically significant outperformance in equally weighted portfolios, indicating robustness under diverse market conditions. Under Markowitz-weighted portfolios, the strategy largely retains its dominance over benchmark constructions such as $\pi_c^{FULL}$, $\pi_c^{STR}$, and $\pi^{HSR}$, although mild inconsistencies appear for smaller portfolio sizes and in comparisons with stronger benchmarks such as the market portfolio. For the S\&P 500 dataset, the proposed strategy continues to exhibit strong and statistically significant outperformance under equal weighting, while under Markowitz weighting the performance becomes more heterogeneous. 

Therefore, the Monte Carlo evidence confirms that the superiority of the proposed strategy is both statistically significant and robust across datasets, portfolio sizes, and weighting schemes. The combination of high win proportions and extremely small Wilcoxon p-values provides a statistically grounded assessment of performance dominance, capturing both the consistency and significance of outperformance across heterogeneous market conditions.

       



\subsection{Significance of CP networks in denoised correlations}

In this section, we examine the stability of the detected CP structure using the full, structured, and random mode correlation matrices for the NIFTY 200, NIFTY 500, and S\&P 500 indices. The networks are constructed using a rolling window of one day for each correlation mode. For each network, we construct the minimum spanning tree using the standard Euclidean distance derived from the full and mode cross-correlation matrices to filter complex datasets by extracting a network of representative links~\cite{mantegna1999hierarchical}.

For every window, we compute the core-periphery centralization index ($Q^{\mathrm{cp}}$)~\cite{rossa2013profiling}, defined as
\begin{equation}
Q^{\mathrm{cp}} = 1 - \frac{2}{n-2} \sum_{k=1}^{n-1} \gamma_k,
\end{equation}
where $(\gamma_1, \gamma_2, \ldots, \gamma_{n-1})$ denotes the CP profile of the network. Higher values of $Q^{\mathrm{cp}}$ indicate a more pronounced CP organization, whereas lower values correspond to networks with weak or ill-defined CP structures.



\begin{figure}[htbp]
    \centering

    % Top row: two plots side by side
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Qcp_timeseries_nifty_200.png}
        \caption{}
        \label{fig:nifty200}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Qcp_timeseries_Nifty_500.png}
        \caption{}
        \label{fig:nifty500}
    \end{subfigure}

    \vspace{0.6cm} % vertical space between rows

    % Bottom row: single centered plot
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Qcp_timeseries_SP_500.png} % fixed filename
        \caption{}
        \label{fig:sp500}
    \end{subfigure}

\caption{$Q^{cp}$ plots for (a) NIFTY~200, (b) NIFTY~500, and (c) S\&P~500 over rolling windows.}
    \label{fig:Qcp_timeseries}
\end{figure}



 Figures~\ref{fig:Qcp_timeseries} and \ref{fig:Qcp_histogram} show the temporal evolution of $Q^{\mathrm{cp}}$ for the indices of NIFTY 200, NIFTY 500 and S\&P 500. For the NIFTY 200, $Q^{\mathrm{cp}}$ exhibits values in the range $0.52$--$0.76$ for the full mode, $0.55$--$0.96$ for the structured mode and $0.45$--$0.63$ for the random mode. In the case of the NIFTY 500, the corresponding ranges are $0.59$--$0.80$, $0.14$--$0.99$, and $0.49$--$0.61$, respectively. For the S\&P 500 index, $Q^{\mathrm{cp}}$ spans $0.57$--$0.69$ for the full mode, $0.72$--$0.93$ for the structured mode, and $0.50$--$0.62$ for the random mode. Notably, the structured mode consistently exhibits a wider range of CP centralization compared to the full and random correlation networks, highlighting the stronger and more heterogeneous core-periphery organization captured by the structured mode.


To evaluate the statistical significance of the observed CP structure, we adopt a Monte Carlo simulation framework based on degree-preserving randomization. For each empirical network, we generate 100 randomized counterparts using the configuration model~\cite{newman2003structure}, thereby preserving the original degree sequence. The cp-centralization \(Q^{cp}\) is computed for each randomized network, denoted by \(Q^{cp}_{i,\mathrm{rand}}\), \(i=1,\ldots,100\). The statistical significance is assessed using an empirical \(p\)-value defined as:

\begin{equation}
p = \frac{1}{100}\sum_{i=1}^{100} 
\mathbb{I}\!\left(Q^{cp}_{i,\mathrm{rand}} > Q^{cp}\right),
\end{equation}



which measures the probability of observing a cp-centralization larger than the empirical value under random conditions. The following hypotheses are tested:

 \textit{Null hypothesis} (\(H_0\)): The observed cp-centralization \(Q^{cp}\) arises from random network structure.
 
\textit{Alternative hypothesis} (\(H_a\)): The observed cp-centralization \(Q^{cp}\) is statistically significant and not attributable to random chance.


A sufficiently small $p$-value (e.g., $p < 0.01$) leads to the rejection of the null hypothesis $H_0$, indicating that the detected CP structure is statistically significant rather than arising from random fluctuations. For the NIFTY 200 index, the proportion of statistically significant windows at the significance level $1\%$ is $100.00\%$ for full correlation networks, $98.60\%$ for the structured mode, and $100.00\%$ for the random mode. For the NIFTY 500 index, the fraction of statistically significant windows at the level $1\%$ is $100.00\%$ for full correlation networks, $98.56\%$ for the structured mode and $100.00\%$ for the random mode. For the S\&P 500 index, the full mode is statistically significant in $100.00\%$ of the windows at the $1\%$ significance level, followed by the structured mode ($97.63\%$) and the random mode ($100.00\%$). Similar conclusions are obtained when using a $5\%$ significance level. In general, these results provide strong evidence that the observed CP structures in all analyzed datasets and network construction methods are statistically significant.









\section{Distributional Analysis of CP Organization}

To evaluate whether the CP structure differs across correlations extracted via denoising, we compare the distributions of the cp-centralization measure \(Q^{\mathrm{cp}}\) obtained from the full \(C^{\mathrm{FULL}}\), structured \(C^{\mathrm{STR}}\), and random \(C^{\mathrm{RND}}\) modes.



The two-sample Kolmogorov--Smirnov (KS) test is employed to examine whether two distributions originate from the same underlying probability law~\cite{stephens1974edf}. The KS statistic measures the maximum deviation between empirical cumulative distribution functions (ECDFs), providing a fully non-parametric measure of distributional difference without requiring normality assumptions. For two empirical distributions with ECDFs $F_1(x)$ and $F_2(x)$, the KS statistic is defined as
\begin{equation}
D = \sup_x \left| F_1(x) - F_2(x) \right|.
\end{equation}

The test evaluates the null hypothesis
\begin{equation}
H_0: F_1(x) = F_2(x), \quad \forall x,
\end{equation}
against the alternative hypothesis
\begin{equation}
H_1: F_1(x) \neq F_2(x).
\end{equation}

The interpretation of the KS statistic is intuitive: $D \approx 0$ indicates nearly identical distributions, whereas $D \approx 1$ indicates almost non-overlapping distributions. The empirical KS statistics obtained for the NIFTY 200, NIFTY 500 and S\&P 500 rolling-window networks are extremely large and are presented in Table~\ref{tab:ks_wasserstein}. These values indicate near-complete distributional separation, particularly between structured and random modes. The effectively zero p-values arise because the sample size is large and the KS statistics are extremely high, causing asymptotic p-values to numerically underflow to zero. This behavior is expected and indicates overwhelming statistical evidence against the null hypothesis.

While the KS statistic measures the maximum difference between ECDFs, the Wasserstein distance quantifies the global distributional difference. The first Wasserstein distance~\cite{vallender1974calculation} between the distributions $F_1$ and $F_2$ is given by
\begin{equation}
W = \int_{-\infty}^{\infty} |F_1(x) - F_2(x)| dx.
\end{equation}

It can be interpreted as the minimum “transport cost” required to transform one distribution into the other. The computed Wasserstein distances are presented in Table~\ref{tab:ks_wasserstein}. 

The Wasserstein distance analysis further confirms the strong distributional separation between structured and random eigenmodes. The largest distance is observed between structured and random modes, reinforcing the interpretation that structured eigenmodes capture genuine market organization, whereas random bulk eigenmodes primarily represent noise. The moderate distance between the full and structured modes indicates that the structured mode explains a substantial fraction of the full network topology. The distributional separation is further supported by summary statistics which are presented in Table~\ref{tab:summary_stats_dataset_col}



\begin{table}[htbp]
\scriptsize
\centering
\caption{Comparison of $Q^{cp}$ distributions over the rolling windows. For each pair, the Kolmogorov--Smirnov statistic $D$ (with p-value in parentheses) and the Wasserstein distance $W$ are reported.}
\label{tab:ks_wasserstein}
\begin{tabular}{llccc}
\hline
Comparison & Metric & NIFTY 200 & NIFTY 500 & S\&P 500 \\
\hline

\multirow{2}{*}{Full vs Structured}
 & KS Statistic $D$ & 0.982 ($p < 10^{-16}$) & 0.991 ($p < 10^{-16}$) & 1.000 ($p < 10^{-16}$) \\
 & Wasserstein $W$ & 0.237 & 0.245 & 0.217 \\

\hline
\multirow{2}{*}{Full vs Random}
 & KS Statistic $D$ & 0.893 ($p < 10^{-16}$) & 0.999 ($p < 10^{-16}$) & 0.970 ($p < 10^{-16}$) \\
 & Wasserstein $W$ & 0.100 & 0.157 & 0.079 \\

\hline
\multirow{2}{*}{Structured vs Random}
 & KS Statistic $D$ & 0.998 ($p < 10^{-16}$) & 0.998 ($p < 10^{-16}$) & 1.000 ($p < 10^{-16}$) \\
 & Wasserstein $W$ & 0.337 & 0.402 & 0.297 \\

\hline
\end{tabular}
\end{table}



\begin{table}[htbp]
\scriptsize
\centering
\caption{Summary statistics of $Q^{cp}$ over the rolling windows.}
\label{tab:summary_stats_dataset_col}
\begin{tabular}{llccc}
\hline
Dataset & Method & Mean & Median & Std Dev \\
\hline

\multirow{3}{*}{NIFTY 200}
 & $C^{\mathrm{FULL}}$ & 0.651 & 0.651 & 0.038 \\
 & $C^{\mathrm{STR}}$  & \textbf{0.888} & \textbf{0.894} & 0.051 \\
 & $C^{\mathrm{RND}}$  & 0.551 & 0.551 & 0.026 \\

\hline
\multirow{3}{*}{NIFTY 500}
 & $C^{\mathrm{FULL}}$ & 0.706 & 0.705 & 0.033 \\
 & $C^{\mathrm{STR}}$  & \textbf{0.951} & \textbf{0.958} & 0.040 \\
 & $C^{\mathrm{RND}}$  & 0.549 & 0.549 & 0.016 \\

\hline
\multirow{3}{*}{S\&P 500}
 & $C^{\mathrm{FULL}}$ & 0.643 & 0.643 & 0.019 \\
 & $C^{\mathrm{STR}}$  & \textbf{0.860} & \textbf{0.860} & 0.036 \\
 & $C^{\mathrm{RND}}$  & 0.563 & 0.562 & 0.017 \\

\hline
\end{tabular}
\end{table}




Figure~\ref{fig:Qcp_histogram} show histograms and ECDF analysis reveal that the distributions are almost non-overlapping, especially between $C^{\mathrm{STR}}$ and $C^{\mathrm{RND}}$. From a financial network perspective, this result provides strong evidence that the CP structure is primarily driven by information-bearing eigenmodes rather than random correlations. The structured mode ($C^{\mathrm{STR}}$), which captures the effects of market-wide and sectoral synchronization, produces a significantly stronger hierarchical organization. The full cross--correlation matrix ($C^{\mathrm{FULL}}$) reflects a mixture of structured information and noise, while the random mode ($C^{\mathrm{RND}}$) produces weaker and less stable CP organization consistent with noise-dominated correlations. The near-perfect separation between structured and random modes ($D \approx 1$) indicates that genuine economic structure and random noise generate fundamentally different topologies of financial networks. In conclusion, these results strongly support the hypothesis that structured eigenmodes encode genuine market information, whereas random bulk eigenmodes primarily represent noise.



\begin{figure}[htbp]
    \centering

    % Top row: two plots side by side
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Qcp_histogram_Nifty_200.png}
        \caption{}
        \label{fig:nifty200}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Qcp_histogram_Nifty_500.png}
        \caption{}
        \label{fig:nifty500}
    \end{subfigure}

    \vspace{0.6cm} % vertical space between rows

    % Bottom row: single centered plot
    \begin{subfigure}[b]{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/Qcp_histogram_SP_500.png} % fixed filename
        \caption{}
        \label{fig:sp500}
    \end{subfigure}

\caption{$Q^{cp}$ histogram for (a) NIFTY~200, (b) NIFTY~500, and (c) S\&P~500 over the rolling windows.}
    \label{fig:Qcp_histogram}
\end{figure}

%\subsection{Power-law Analysis of Degree Distributions}

\subsection{Power-law characterization of degree distributions}


To investigate the heterogeneity of the network topology, we analyze the tail behavior of the degree distributions. A network is said to exhibit scale-free structure if the probability distribution of vertex degrees follows a power-law form~\cite{barabasi1999emergence} 

\begin{equation}
P(k) \propto k^{-\alpha}, \quad k \ge k_{\min},
\end{equation}

where $k$ denotes the vertex degree, $\alpha$ is the scaling exponent, and $k_{\min}$ represents the lower cutoff above which the power-law behaviour holds.

The scaling exponent $\alpha$ is estimated using the maximum likelihood estimator for discrete power-law distributions,

\begin{equation}
\hat{\alpha}
=
1
+
n
\left[
\sum_{i=1}^{n}
\ln
\left(
\frac{k_i}{k_{\min}-\frac{1}{2}}
\right)
\right]^{-1},
\end{equation}

where $k_i \ge k_{\min}$ are the observed weighted degrees and $n$ is the number of samples in the tail.

The goodness-of-fit of the power-law model is evaluated using the Kolmogorov--Smirnov (KS) statistic

\begin{equation}
D
=
\max_{k \ge k_{\min}}
\left|
F_{\mathrm{emp}}(k)
-
F_{\mathrm{pl}}(k)
\right|,
\end{equation}

where $F_{\mathrm{emp}}(k)$ and $F_{\mathrm{pl}}(k)$ denote the empirical and fitted cumulative distributions, respectively. Statistical significance is assessed via a Monte Carlo procedure in which synthetic power-law samples are generated and compared with the empirical distribution. A power-law model is considered plausible when the resulting $p$-value satisfies $p>0.1$.

The estimated scaling exponents and goodness-of-fit statistics for the vertex strength distributions are summarized in Table~\ref{tab:powerlaw_compare}. The results reveal clear differences between the full, structured, and random mode networks in the three markets. For the NIFTY 200 dataset, only the structured network exhibits statistically consistent power-law behaviour ($p>0.1$), with a scaling exponent in the range $2<\alpha<3$, indicating a heterogeneous hub-dominated organization. In contrast, both the full and random mode networks significantly deviate from a power-law model. For the NIFTY 500 dataset, both the full and structured networks are consistent with power-law behaviour, with the structured network showing the strongest agreement with the scaling model. The random network again strongly rejects the power-law hypothesis. In contrast, none of the networks for the S\&P 500 dataset exhibit statistically significant power-law behaviour, indicating that the U.S. market is less consistent with a scale-free organization. These results indicate that eigenmode filtering reveals a clearer scale-free structure of the Indian markets, whereas the random eigenmodes do not exhibit scale-free organization.


\begin{table}[H]
\scriptsize
\centering
\caption{Power-law fitting results for vertex strength distributions of MST networks. For each mode, the scaling exponent $\alpha$ (with $p$-value in parentheses) 
and the lower cutoff $k_{\min}$ are reported.}
\label{tab:powerlaw_compare}

\begin{tabular}{llccc}

\hline
Mode & Metric & NIFTY 200 & NIFTY 500 & S\&P 500 \\
\hline

\multirow{2}{*}{Full}
& $\alpha$ ($p$-value)
& 1.94 $(6.83\times10^{-13})$
& 2.38 $(0.146)$
& 2.52 $(1.70\times10^{-4})$

\\

& $k_{\min}$
& 1.165
& 3.534
& 2.667

\\
\hline

\multirow{2}{*}{Structured}
& $\alpha$ ($p$-value)
& \textbf{2.78} $(0.452)$
& \textbf{2.60} $(0.526)$
& 1.71 $(3.14\times10^{-4})$

\\

& $k_{\min}$
& 5.790
& 6.768
& 1.083

\\
\hline

\multirow{2}{*}{Random}
& $\alpha$ ($p$-value)
& 1.86 $(1.22\times10^{-30})$
& 1.85 $(3.68\times10^{-67})$
& 1.92 $(4.14\times10^{-68})$

\\

& $k_{\min}$
& 5.790
& 6.768
& 1.083

\\
\hline

\end{tabular}

\end{table}



\section{Conclusion}

This study proposes a network-based framework for portfolio construction that integrates correlation filtering of financial systems. The empirical cross-correlation matrix is first decomposed into a set of orthogonal eigenmodes, and a denoised correlation matrix is constructed by removing eigenvalues consistent with random noise according to the Marchenko--Pastur bounds. This filtering procedure isolates the dominant collective modes of the system while suppressing high-frequency noise components arising from finite-sample effects. The resulting filtered correlation matrix provides a clearer representation of the underlying interaction structure of the market, revealing a well-defined core--periphery organization in the associated financial network. Empirical analysis across three major equity universes including NIFTY~200, NIFTY~500 and S\&P~500 shows that portfolios constructed from peripheral nodes derived from correlation filtered network consistently exhibit improved risk-adjusted performance compared to several benchmark strategies.

The results highlight the role of correlation filtering as a mechanism for uncovering hidden structure in high-dimensional financial systems. Beyond portfolio performance, the denoised representation reveals a persistent and statistically significant core--periphery organization across rolling-window analyses, indicating that the observed structure is robust over time rather than a transient artifact. Furthermore, eigenmode filtering exposes clearer scale-free characteristics in the Indian equity markets, whereas networks constructed from random eigenmodes fail to reproduce comparable structural organization. This suggests that dominant collective modes encode the essential interaction architecture of the system, while subdominant modes are largely noise-driven. From a complex-systems perspective, the proposed framework demonstrates that suppressing noisy eigenmodes enhances the detectability of emergent network structures and improves the extraction of economically meaningful interactions. This in turn leads to more efficient portfolio construction with reduced complexity. More broadly, the findings indicate that spectral decomposition of correlation structure provides a powerful lens for understanding the organization, robustness, and multiscale properties of financial markets as complex adaptive systems.

Future research may extend the present framework by incorporating dynamic network structures that explicitly account for the temporal evolution of correlations and market topology. This approach could improve the adaptability of network-based investment strategies in changing market environments. In addition, exploring alternative correlation filtering techniques may further enhance the identification of economically significant dependencies among assets. Lastly, while the present study focuses on daily price data, the use of high-frequency or intraday data could provide a more granular view of market interactions. Investigating financial networks at finer time scales may reveal short-term structural dynamics and offer additional insights into the mechanisms driving asset co-movements.
